OpenVPN is Open to VPN Fingerprinting

VPN adoption has seen steady growth over the past decade due to increased public awareness of privacy and surveillance threats. In response, certain governments are attempting to restrict VPN access by identifying connections using "dual use" DPI technology. To investigate the potential for VPN blocking, we develop mechanisms for accurately fingerprinting connections using OpenVPN, the most popular protocol for commercial VPN services. We identify three fingerprints based on protocol features such as byte pattern, packet size, and server response. Playing the role of an attacker who controls the network, we design a two-phase framework that performs passive fingerprinting and active probing in sequence. We evaluate our framework in partnership with a million-user ISP and find that we identify over 85% of OpenVPN flows with only negligible false positives, suggesting that OpenVPN-based services can be effectively blocked with little collateral damage. Although some commercial VPNs implement countermeasures to avoid detection, our framework successfully identified connections to 34 out of 41 "obfuscated" VPN configurations. We discuss the implications of the VPN fingerprintability for different threat models and propose short-term defenses. In the longer term, we urge commercial VPN providers to be more transparent about their obfuscation approaches and to adopt more principled detection countermeasures, such as those developed in censorship circumvention research.

==> design.tex <==
\section{Threat Model and System Design}
\label{sec:design}


In this paper, we will attempt to explore how \textit{practical} it is to fingerprint OpenVPN as well as its obfuscated variants while adopting the viewpoint of ISPs and censors. We first note that due to the limited study on real-world censors exploiting vulnerabilities of circumvention tools, a realistic censor capability model remains unclear to the community~\cite{sok-obfs}. We build our threat model based on the assumed capabilities of censors and ISPs (referred to as ``adversary’’) based on knowledge from previous measurement studies on the arms race between censors and circumventors~\cite{how-china-detect-shadowsocks, how-china-detect-tor, sok-obfs, Ensafi-active-probing}.

We assume the adversary operates a two-step detection pipeline, which has been adopted by real-world censors such as the GFW against Tor~\cite{Ensafi-active-probing, how-china-detect-tor}. In the first step, we outline an on-path adversary who is able to passively observe and examine passing network traffic. The adversary is stateful, but has limited resources and can maintain a limited amount of per-connection states for a short amount of time. The adversary also has smaller long-term data storage and computation resources, which may restrict it from performing machine learning at line speed.
%These conditions should be reasonable for most ISPs, and censors.
We also expect that the adversary is familiar with the OpenVPN protocol and has access to the different obfuscators deployed by VPN providers (i.e., as a paid customer). %We assume the adversary can generate an OpenVPN-specific fingerprint based on its observation of traffic features such as raw packet content or packet length. 

For the second step of the pipeline, we assume that the adversary records the server IP and port numbers for the suspected flows from the previous step. The adversary can then asynchronously feed these IP and ports to a distributed probing system to perform follow-up probing in order to confirm their detection results. We note that while the adversary may be able to enumerate all available servers as a paid customer, we consider obtaining a complete list of server IPs belonging to a specific provider outside the scope of this paper.

%\input{figures/design}
\input{figures/deployment}

Based on such a threat model, we implement a system prototype inside the \textit{Merit} Network, as shown in Figure~\ref{fig:deployment}. The first step involves a \textit{Filter} (Monitoring Station) performing cheap, passive filtering over mirrored network traffic. For each suspect flow, the Filter logs its server IP and port information into a database. The second part is a distributed system containing \textit{Probers}, located inside a University network. The \textit{Probers} periodically retrieve lists of targets and perform follow-up probing to confirm if they are running suspected protocols. Once confirmed, connections to the server IP and port and the user making these connections can be identified and can be logged, throttled, or blocked, according to the adversary's policy. In the next two sections, we detail our design of the \textit{Filter} and \textit{Prober}.

==> figures/design.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth,keepaspectratio]{figures/design.png}
\caption{Two-phase system design based on threat model}
\label{fig:design}
\end{figure}

==> figures/loss.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth,keepaspectratio]{figures/loss.png}
\caption{\textbf{Test results under different loss rate.}\TODO{Redo figure}}
\label{fig:loss}
\vspace{-15pt}
\end{figure}

==> figures/observation-N.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth,keepaspectratio]{figures/N.png}
\caption{\textbf{Filtering results from different observation windows.}}
\label{fig:observation-N}
\vspace{-15pt}
\end{figure}

==> figures/subnet.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth,keepaspectratio]{figures/subnet.png}
\caption{Probing adjacent IPs of known OpenVPN servers}
\label{fig:subnet}
\end{figure}

==> figures/timeout.tex <==
\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth,keepaspectratio]{figures/timeout.png}
\caption{CDF for OpenVPN Server Handshake Window}
\label{fig:timeout}
\end{figure}

==> filter.tex <==
%\section{Filter}
\section{Fingerprinting Feature Extraction}
\label{sec:Filter}
To detect OpenVPN we need to understand what features in the protocol makes it vulnerable to fingerprinting by a real-world adversary. We identify and extract three features targeting byte pattern, packet length, and server behaviors, respectively.


We design \textit{Filters} exploiting two features distinct to OpenVPN: \textit{Opcodes} and \textit{ACK Packets}. Both features are fingerprintable for vanilla OpenVPN configurations and they each targets a specific subset of obfuscation layers: the former works against XOR-based obfuscations that work like Vigenère ciphers, \ie they always encrypt the same plaintext opcodes at the same position to the same ciphertext bytes, whereas the latter works against tunneling-based obfuscation that lacks random padding and preserves the 1:1 correspondence between the original and obfuscated packet streams.

We implement the \textit{Filters} in Zeek, an open-sourced network security monitoring tool~\cite{Zeek}. We note that the evaluation processes for both \textit{Filters} are quite simple: both of them only require several dozens of integer comparison limited by the observation window while maintaining a small number of per-flow states. We therefore believe that they can be easily deployed by any ISP or censor. 

\subsection{Dataset}

We use two datasets in this section to explore features of OpenVPN traffic as well as to quantify thresholds for detection (\eg number of packets to see before making a verdict). 

\paragraph{ISP Dataset} We collected a snapshot of network traffic going through a server installed within \textit{Merit}. Over 45 minutes on July 28, 2021, we sampled 1/30 of all flows passing through the server, resulting in 461~GB of traffic that corresponds to 221,534 flows with full packet payloads.

\paragraph{VPN Dataset} We collected traces from 20 commercial VPN providers as well as 2 self-hosted OpenVPN services (Streisand, OpenVPN Access Server) following an automated process described in Section~\ref{sec:setup}. Note the 20 providers do not overlap with the providers used in evaluation. For each provider, we repeated the trace collection process 50 times each in TCP and UDP mode, resulting in a 7.65~GB dataset comprised of 2,200 VPN traces.

\input{filter-algo}

\subsection{Opcode-based Fingerprinting}
%\subsection{Filtering by Opcodes}
Each OpenVPN packet has a header of 24 bits under TCP mode or 8 bits under UDP mode, which is not part of the encrypted payload and is transmitted in plaintext. Each OpenVPN header starts with an opcode that specifies the message type of the current packet and a key ID that refers to a (new) TLS session. The opcode field can take over 10 defined values, corresponding to message types transmitted during different communication stages. A typical OpenVPN session starts by client sending a \texttt{Client Reset} packet. The server, upon receiving this packet, responds with a \texttt{Server Reset} packet, and a TLS handshake follows. OpenVPN packets that carry TLS ciphertexts have \texttt{P_Control} as their message type. Since OpenVPN can run over UDP but it has to provide a reliable channel for TLS, each \texttt{P_Control} packet is explicitly acknowledged by \texttt{P_ACK} packets (not to be confused with TCP ACK packets). Finally, actual payloads are transmitted in packets typed as \texttt{P_Data}. Figure~\ref{fig:negotiation} illustrates this sequence of packet exchange annotated with opcodes.

We fingerprint this unique handshake process by analyzing the opcode bytes presented in the first N packets of a flow (the threshold for N is explored in Section~\ref{sec:Observation-Window}). 
%While previous work and currently deployed open-sourced DPI tools~\cite{Pang2012OpenVPNTI, nDPI, libprotoident, Zeek-OpenVPN} detect OpenVPN flows based on static signatures, we design our heuristic to be more generic and flexible in order to cover XOR-based obfuscation variants while still keeping the filter selective enough to keep the list of probing candidates short. 
Algorithm 1 shows the evaluation process of opcode fingerprinting. \texttt{Opcode[i]} refers to the byte value at the Opcode position from the $i^{th}$ packet of a given flow. Briefly, the filter flags a flow as suspected OpenVPN if the number of different opcodes observed accords with the protocol \textit{and} the Client and Server Reset are not observed once the handshake process has been completed.

\input{figures/xor-reverse}

%\input{tables/dpi-comparison}
%Table~\ref{tab:dpi-comparison} compares our heuristics with those used in previous works and existing open-sourced DPI tools. 
Compared with previous works or existing open-source DPIs~\cite{ndpi, Zeek, libprotoident, OpenVPN-Opcode}, our heuristics do not require exact matching of opcode values or packet length (\eg, does not require the third byte of the first packet to be b'x38'), thereby ensuring it works effectively against XOR-obfuscated flows. The XOR obfuscation masks packet payloads to ensure that the opcode bytes are altered. Notably, according to the specification~\cite{OpenVPN-XOR}, when it reverses the packet as one of the obfuscation steps, it excludes the first character of the buffer from reversion, as shown in Figure~\ref{fig:xor-reverse}. As such, the opcode bytes are always XOR-ed with the same byte of the XOR key, and the same opcodes would be mapped to the same value after obfuscation. This behavior is preserved when Tunnelblick adopts the patch (``for interoperability''~\cite{Tunnelblick-XOR}), and has been adopted by multiple mobile apps~\cite{Zhang2017OhPwnVPNSA}. By considering only the number of unique opcodes seen so far, our heuristics are more flexible and targets various XOR-based obfuscated OpenVPN.

\subsection{Ack-based Fingerprinting}

Since TLS is designed to operate over a reliable layer, OpenVPN implements an explicit acknowledgement and re-transmission mechanism for its control channel messages. This is especially important when OpenVPN is running over UDP~\cite{openvpn-reliable}. Specifically, incoming \texttt{P_Control} packets are acknowledged by \texttt{P_ACK} packets, which do not carry any TLS payloads and are uniform in sizes. %(Note these ACK packets are carried over by TCP as payload and are not the same as TCP ACK flags.)
Moreover, these ACK packets are seen mostly only in the early stage of a flow, during the handshake phase, and are not used in the actual data transfer channel, which can run over an unreliable layer.%(Later in the session, Control and ACK packets can be exchanged again to transfer random key materials, but it is not expected to be observed within our observation window N).
%These ACK packets, uniform in size and only seen in some parts of a session, provide another fingerprintable feature that is unique to the OpenVPN protocol.

The existence of ACK packets provide another fingerprintable feature unique to the OpenVPN protocol. Specifically, we first identify a likely ACK packet of a session by locating a reset packets exchange sequence of C->S (Client-Reset), S->C (Server-Reset), C->S (ACK), C->S (Control). For vanilla OpenVPN, XOR-based obfuscation, or 0-RTT obfuscator (\eg, Shadowsocks), the first ACK packet usually appears as the third (data) packet transmitted in a session. For tunnels that have their own handshake or key exchange process (\eg, Stunnel, SSH tunnel, or Obfsproxy), this counting is offset by the number of tunnel handshake packets. Next, we group packets into 10-packet bins, and we derive the ACK fingerprint for each flow by counting the number of packets in each bin that have the same size as the identified ACK packet. This approach proves effective to fingerprint vanilla OpenVPN as well as obfuscated services running over encrypted tunnels that lack random padding. 

\input{figures/ack-dt}
%\input{figures/ack-bin}
\input{tables/ack-fingerprint}

We derive ACK fingerprints for the ISP and VPN datasets. We only include flows with at least 150 data packets (15 bins), which leaves us with 24069 ISP flows and 2200 flows from the VPN dataset. A classification decision tree is constructed based on the two (labeled) sets with weights applied to account for the imbalanced data size. Figure~\ref{fig:ack-dt} presents the constructed tree (depth and leaf limited, a complete graph can be found in Appendix~\ref{sec:ack-tree}). The ACK fingerprint is a set of thresholds based on the derived decision tree, as shown in Table~\ref{tab:ack-fin}. ($Bin[i]$ refers to the number of ACK-size packets for $i^{th}$ Bin.)

%\begin{itemize}
  %\item $1 \leq Bin[1] \leq 3$
  %\item $2 \leq Bin[2] \leq 5$
  %\item for $i$ in range $[3, 5]$, $Bin[i] \leq 5$
  %\item for $i$ in range $[6, N/10]$, $Bin[i] \leq 1$
%\end{itemize}

%Figure~\ref{fig:ack-bin} shows ACK fingerprints for the two datasets as well as the thresholds generated from the decision tree.

\section{Fine-tuning for Deployment}
So far we described a specific features in openvpn handshake and payload that can help with detecting openvpn traffic . In real world detection, there are metrics that can affect the accuracy or precision or anything else such as packet loss etc.

\subsection{Determining an Observation Window N}
\label{sec:Observation-Window}

Previous works attempt to identify VPN traffic only \textit{after} the flow terminates, as they make use of aggregated statistics such as connection duration~\cite{Deep-Packets, VPN-nonVPN, perceptron-nn-VPN}. However, detecting disallowed traffic only after the flow is finished may be of very limited interest to a real-world censor~\cite{On-the-fly}. We therefore have two objectives for our \textit{Filter}: to be as selective as possible to ensure the subsequent step has less targets to probe, \textit{and} to detect OpenVPN as soon as possible within a flow. %These two goals can be at odds with each other: intuitively, the more packets we observe, the more confident we can be about our filtering results.


Inspired by~\cite{On-the-fly, detect-obfuscation}, we consider the windowing strategy of limiting the inspection to only the first N data packets of a flow. We tested N from \{10, 20, 30, ..... 200\} on the ISP and VPN dataset. As shown in Figure~\ref{fig:observation-N}, the number of flows from ISP dataset that pass the \textit{Filters} declines from over 62000 to 322 as we extend the observation window. However, an observation window of 100 packets has already achieved a precision within 2\% of the best performing (200 packets). Therefore, in this work we use 100 packets as the observation window in order to get a timely and accurate detection.

\input{figures/observation-N}

\subsection{Effects of packet loss on filtering results}

\input{figures/loss}
We investigate the effects of packet loss on the performance of the filters. All our previous tests were offline, by configuring Zeek to read from pre-collected packet captures. In such settings, Zeek can take as long as necessary to process the capture. 

%Due to the nature of the opcode filter, we need to inspect the raw contents of each and every reassembled packet of any suspect flow, until the observation window is reached. All traffic must be passed on to Zeek's scripting layer, which affects the performance of the system and leads to a CPU bottleneck. When we did attempted to process all traffic arriving at the server, we ran into massive packet loss as high as 70\%. 
%However, an adversary monitoring a busy network needs to keep pace with the packet arrival rate, or otherwise packet drops will start to occur due to CPU bottleneck. For example, we collected the ISP dataset by sampling 1/30 flows over 45 minutes on \textit{Merit} Network. Yet, it takes Zeek over 2 hours to process the collected packet capture in a single-thread setting. The main reason is that the opcode filter needs to inspect the raw contents of each and every reassembled packet of any suspect flow, until the observation window is reached. This means that all traffic must be passed on to Zeek's scripting layer, which leads a CPU bottleneck. On the \textit{Merit} server monitoring two 10 GB interfaces, processing all traffic without sampling can lead to substantial packet loss as high as 70\%. In addition to CPU bottleneck, Network Interface Card (NIC) may also become an upstream bottleneck and leads to end-to-end packet loss. We therefore explore what to expect from our filters when packet loss is inevitable.

%We configure Zeek to ignore events signaling new packets with different probabilities in order to simulate random packet loss. We tested different loss rates from 1\% up to 80\%. For each test, we count it as a positive result if either ACK or Opcode filter flags the flow as suspect flow. The experiment was repeated three times and average results reported in Figure~\ref{fig:loss}. We find that packet loss starts to have noticeable effects on the filters' outputs once the loss rate surpasses 10\%. Therefore, in order to minimize the effects of packet loss, for all following online tests and evaluations, we always configure the monitor to sample flows with a given rate (adjusted with CPU resources and traffic volume).

\section{Fingerprint Preliminary Evaluation}
\subsection{Test the \textit{Filters} on live traffic}

We test how selective the two \textit{Filters} are by running them in an online setting. From 14:00 EDT on August 2, 2021, we ran our Zeek filters on a monitoring server inside \textit{Merit} for 24 hours. To minimize the effects of packet loss, we sampled 10\% of passing traffic (at the flow level) and fed traffic to a 15-worker Zeek cluster. The packet loss rate was kept below 3\% on average. (Please refer to Appendix~\ref{sec:loss} for a discussion on the effect of packet loss, where we show that frequent packet loss can lead to \textit{underblocking} but not \textit{overblovking}, which is favoured by real-world censors.)

As shown in Table~\ref{tab:filter-prober}, the \textit{Filters} are highly selective: from over 1.6 million flows that exceeded the Observation Window of 100 packets, it labels 10935 flows as OpenVPN suspects, drastically shrinking down probing targets by 99.3\%. However, at this step, there was no attempt to further validate these results as true or false positives. Results from \textit{Filters} are followed up by active probing, and only the false positives of both steps are the true potential collateral damage of fingerprinting OpenVPN traffic.

%\subsection{Summary}
%Our manually-created Opcode fingerprints and the ACK-size decision tree detects an OpenVPN flow in its handshake stage based on our observations of the OpenVPN protocol and its packet structures. In addition, these two filters also attempt to capture OpenVPN flows with obfuscations by exploiting either obfuscator's insufficient encryption or lack of random padding. We note that the evaluation process of the Opcode fingerprints and the ACK decision tree is quite simple: both of them only require several dozens of integer comparison limited by the observation window chosen while maintaining a small number of per-flow states. We therefore believe that the filters can be relatively easy to deploy by a resourceful ISP or censor.

==> prober.tex <==
%\section{Prober}
\section{Active Server Fingerprinting}
\label{sec:Prober}

Although \textit{Filters} have low positive rates of less than 1\%, due to the low base rate of VPN traffic, the majority of flows detected could still be false positives~\cite{detect-obfuscation}. This makes it less practical to real world adversaries who are sensitive to false blocking and collateral damages. We therefore append the filtering phase with a more expensive, but also more accurate follow-up probing stage: the \textit{Prober} extracts IP and port information from suspected flows, and then asynchronously sends a set of predefined probes to the targets in order to confirm if it is an OpenVPN server. This technique has been heavily used by the Great Firewall of China against various censorship circumvention tools, such as Tor or Shadowsocks~\cite{Ensafi-active-probing, how-china-detect-shadowsocks, how-china-detect-tor}.

\subsubsection{OpenVPN goes silent}

A major obstacle to actively fingerprinting OpenVPN servers is the \textit{tls-auth} and \textit{tls-crypt} options~\cite{tls-auth}. These options, which have been adopted by most commercial providers, add an additional HMAC signature---signed by a pre-shared key---to every control channel packet for integrity verification, including the initial client/server reset packets. With either of these option enabled, an OpenVPN server would not respond to unauthenticated client reset with server reset, but would silently drop such packets without further processing. 
%From the official documentation, these options protect servers from active port scanning, among other security benefits~\cite{tls-auth}. Typically, OpenVPN servers would respond to a client reset with an explicit server reset, thereby giving away their identity. However, servers protected by this HMAC mechanism, which has been adopted by most commercial providers, would only respond to probes after the client proves knowledge of a pre-shared secret.
The presence of such HMAC mechanism increases the complexity of doing active probing: it effectively makes OpenVPN servers ``probe-resistant''~\cite{Frolov-probe-resistant} by making them silent when probed by an unauthenticated client.

In fact, similar HMAC mechanisms are used by more popular ``probe-resistant'' proxies, such as Obfs4~\cite{obfs4}. However, unlike Obfs4 which waits for a server-specific random delay before dropping an unauthenticated connection, OpenVPN always \textit{immediately} closes the connection if a valid HMAC cannot be located. We design our probes leveraging this protocol-specific behavior, and as a result, we manage to fingerprint OpenVPN servers even if they do not respond throughout our probing cycles. The key concept is that although the application may not respond to probing, an attacker may still be able to fingerprint application-specific thresholds at the TCP level, such as timeout or close thresholds~\cite{Frolov-probe-resistant}.

%\input{tables/filter-online}
\input{tables/filter-prober-combined}

\subsubsection{Dataset}
%Two datasets were used in this section to test and improve the accuracy of our active probing scheme.

\paragraph{ZMap Dataset} In an effort to construct a realistic non-VPN endpoints dataset, we used ZMap to scan each of the 65535 TCP ports over the entire IPv4 space for 200 endpoints with the specific port open. This results in a dataset of over 13 million endpoints evenly spread over every TCP ports.

\paragraph{Censys Dataset} We used \texttt{Censys.io}~\cite{censys15} to collect a set of endpoints recognized as running OpenVPN services. From multiple global vantage points, Censys continually scans the Internet on over 2,000 ports, including the official OpenVPN port 1194. We query Censys' database for hosts with TCP port 1194 open. Next, we probe each endpoint with a typical OpenVPN client reset and group endpoints that respond with a server reset. This results in a dataset of 180,858 hosts known to be OpenVPN endpoints (with ``tls-auth'' disabled).

\subsubsection{Base Probes}
\label{sec:probe-scheme}

\input{figures/openvpn-tcp}

The first set of probes aims to exploit a behavior associated with how OpenVPN packetizes TCP streams. When OpenVPN operates over TCP, it needs to split the continuous stream into individual OpenVPN packets.
%Essentially, OpenVPN allocates a buffer to build up packets encapsulated in streams and returns the packet only after it is reassembled.
Figure~\ref{fig:openvpn-tcp} presents a high-level abstraction of this process. The most relevant parts are: a buffer is allocated in memory to read and store fragments of OpenVPN packets encapsulated in TCP streams. The length N for the next OpenVPN packet is extracted from the first two bytes of the OpenVPN TCP header, and the routine keeps reading N additional bytes before it returns the reassembled packet to the caller. This means that an OpenVPN packet will not be parsed and checked for syntax and encryption error before all its parts arrive at the server. 
%The key insight is that the protocol dictates that incomplete packets will not be discarded immediately even if they contain fatal errors (for example, an invalid HMAC signature).

We designed two base probes to trigger an OpenVPN server into different code execution paths, which results in different connection timeouts. As shown in Table~\ref{tab:probes}, the first probe payload is a typical 16-byte OpenVPN \texttt{Client Reset}, while the second probe has the same payload with the last byte stripped off. We sequentially send the first and the second probe to a target and measure the time elapsed before the server responds or terminates the connection. The assumption is since our two probes only differ in one byte, most (Non-OpenVPN) servers will respond to our probes in a similar way. However, for an OpenVPN server with HMAC enabled, the connection sending the first probe will be dropped immediately because the OpenVPN packet is completed and a valid HMAC cannot be located. In contrast, the connection sending the second probe will not receive an immediate response, as the server is waiting for an additional byte to arrive. The connection will stay idle until a server specific handshake timeout has passed, after which the connection will be dropped. As such, the first probe will be dropped at the decryption routine, while the second probe will be dropped at the packet reassembly routine, both labeled red in Figure~\ref{fig:openvpn-tcp}.


\subsubsection{Additional Probes}

The base probes, although useful, are limited and there are other protocols with behaviors similar to OpenVPN. To refine our probing further, we test the base probes on the \textit{ZMap Dataset} by probing endpoints on specific ports and sorting ports based on the number of OpenVPN-like response. For ports with a high number of positive results, we look into the service assigned to that port by IANA. With only two base probes, we still identify a handful of services that respond similarly to OpenVPN servers, such as Microsoft WBT Server (RDP), Message Queuing (MSMQ), and Erlang Port Mapper Daemon (on ports 3389, 1801, 4369 respectively). 

We design additional probes based on the fact that OpenVPN validates packet length and will drop connections sending invalid length without waiting for the next packet to be reassembled. Notice that the packet length here does not refer to the actual TCP packet length but rather the length declared by the first two bytes of an OpenVPN header. A ``valid'' packet length is in the range of [1, \textit{max_len}] bytes where \textit{max_len} is calculated based on server's MTU configurations. For instance, default TUN MTU of 1500 bytes, combined with overheads (crypto IV, packet length, \etc), results in a \textit{max_len} of 1627 bytes. In this case, probes whose first two bytes have a decimal value greater than 1627 (x06x5B) will be dropped immediately.

\input{figures/rst-threshold}
We also designed a probe leveraging the way a Linux server closes a TCP connection. Typically, when a connection terminates, the operating systems at both ends complete a FIN 4-way handshake. However, previous work found that if a connection is closed with unread bytes in buffer, Linux would send a RST packet~\cite{Frolov-probe-resistant}. We conducted binary search on endpoints from the \textit{Censys Dataset} to determine the ``RST Threshold'' of known OpenVPN servers (minimum number of bytes needed to send to the server to trigger a RST). In addition, we search for the same threshold from random Zmap endpoints for comparison. As shown in Figure~\ref{fig:rst-threshold}, the vast majority of OpenVPN servers have a RST threshold around 1550-1660 bytes, corresponding to buffers allocated with typical MTU configurations. In contrast, over 97\% of random endpoints either always ($<500$) or never ($>4000$) RST the connection. We therefore construct an additional probe with 2K random bytes, which we expect over 98\% of legitimate OpenVPN servers and less than 3\% of random servers would respond with RST packets.

%Of the 109115 known OpenVPN endpoints, the largest RST threshold found in the top 20 most common values was 1659 bytes (with 3779 occurrences).

\paragraph{Complication from Port Sharing} OpenVPN provides native support for another application to share its port. This is accomplished by checking whether the first incoming packet has a valid OpenVPN-conforming packet length. If not, the OpenVPN server will forward the packet to the other service sharing the same port. This means that most of our additional probes will be forwarded to and responded by the other application due to invalid packet length. To account for this, we observe that when an OpenVPN shares the port, it is usually shared with either a HTTP, TLS, or SSH server. Therefore, before we send in additional probes, we first send probes targeting these three protocols, and we stop further probing if we get an explicit response for any of these probes. 

It is worth noting that the majority ``typical'' HTTP, TLS, and SSH servers have already been filtered out by our base probes, so endpoints responding to these probes at this stage are likely sharing the port with another service, therefore warranting manual analysis (\eg, checking TLS certificate). On the other hand, while these three services are what we observed, there may be other services running along with OpenVPN, in which case we will not be able to distinguish the server and may lead to false negatives.

Table~\ref{tab:probes} summarizes all probes used and the expected behaviors from an OpenVPN server. A decision tree that illustrates the evaluation process can be found in Appendix. \TODO{ADD TREE} 

\input{tables/probes}
%\subsection{Determining Timeout Threshold}
%We need to calculate a threshold to differentiate between the following two cases: when the server ``immediately'' drops our connection (either due to invalid HMAC or invalid length), versus when the server drops our connection \textit{after} a handshake timeout, because the TLS key negotiation failed to occur. The threshold must be greater than the handshake timeout in order to be able to distinguish the two cases, but also needs to factor in other transient issues such as network delays.

%We used the Censys dataset, which contains 180,858 network hosts that are known to be running OpenVPN servers. We note that these servers do not have the ``tls-auth'' option enabled, which could be different from the majority commercial servers we probed. However, since the ``'tls-auth' option is independent from the ``hand-window'' option, which configures the handshake timeout, we believe the results here are representative of all OpenVPN servers, regardless of whether the HMAC is enabled.

%\input{figures/timeout}
%Figure~\ref{fig:timeout} shows the CDF of handshake timeout configured by the 180,858 OpenVPN servers calculated from our measurement. As expected, most servers do not change the default 60 seconds as the handshake timeout, and majority of the rest servers are configured to timeout in multiples or fractions of minutes. A small group of servers with the shortest handshake timeout are configured to drop connection after 5 seconds if the client fails to authenticate itself. In addition, during our testing, we also found that servers belonging to the OpenVPN's official cloud service (OpenVPN-as-a-service) are also configured to timeout after 5 seconds. We therefore select a distinguishing threshold of 3 seconds and use this for all other tests and evaluations.

%\subsection{Exploring OpenVPN Churn Rate}
%After the \textit{Filter} generates a shorter suspect list, the \textit{Prober} can either send probes synchronously as soon as a target is emitted by \textit{Filter}, or asynchronously, waiting for a pre-configured interval before sending probes to targets in batches. Sending probes synchronously has the advantage of obtaining the most accurate results before the server IP is churned. However, this requires the probing system to be online the whole time. In contrast, sending probes in batches is more efficient and easier to manage, but the server IP may be churned if the interval between filter and prober is excessively long.We explore finding a probing interval and frequency that can balance between efficiency and account for possible server churns. To do this, we monitor the 180,858 OpenVPN servers from the \textit{Censys dataset}. Starting from August 2nd, 18:00 EDT, we probed the servers every 3 hours and recorded their response. Figure~\ref{fig:churn} shows the result.

%\input{figures/churn}
%As we can observe, even after a week, only less than 3\% of OpenVPN servers are either not in the listening state or have been replaced by a different service. This suggests that a majority of OpenVPN servers are not churned frequently. In our evaluation, we choose to configure our system to probe targets on a daily basis, in order to balance between efficiency and potential IP churn. Based on the result of this test, only approximately 0.9\% of servers may be churned within 24 hours.
%we choose to configure our system to probe targets daily and asynchronously, in batches at the end of the day. 

\subsection{Probe UDP and Obfuscated OpenVPN Servers}
\label{sec:probe-subnet}
The aforementioned probing scheme primarily targets vanilla OpenVPN TCP servers, as it exploits the length field within the packet header which is unique to TCP mode that requires packetization. In addition, it works effectively against XOR-obfuscated servers because the XOR encryption is applied to an OpenVPN packet \textit{before} the length field is prepended. This behavior allows us to probe XOR-obfuscated servers in the same way as if they had no obfuscation at all.

In contrast, for UDP or other obfuscated servers, our probes are no longer effective because the length field is either not present (UDP) or is encrypted (tunnel-based obfuscation). However, a critical observation is that most commercial VPN providers usually offer vanilla TCP servers along with UDP and/or obfuscated variants. This is expected as commercial VPN providers attempt to optimize their VPN's performance as well as reliability, since tunnel-based obfuscation adds overhead and UDP traffic may encounter more problems than TCP in a firewalled network. Furthermore, the vanilla TCP service is often co-located with the UDP or obfuscated OpenVPN services, presumably due to lower hosting and maintenance cost. They could be on the same host but listening on different ports, or they could be located in adjacent IPs in the same subnet controlled by the VPN provider. In other words, probing adjacent netblocks of a suspected UDP or obfuscated endpoint may reveal nearby vanilla TCP servers, whose existence corroborates the \textit{Filter} results from the previous step.

%To determine an appropriate subnet size for probing, we use the \textit{Provider Dataset} that contains 439 IPs from 20 commercial VPN providers. For each IP in the list, we used Masscan with a subnet mask N to find all active hosts and their open TCP ports. Next, we probe each host:port following our probing scheme. We repeat this test with different subnet sizes from /32 (65535 ports on the original IP) all the way to /22 (65535 ports for each of the 1024 hosts). 

%However, to probe adjacent IPs determining an appropriate subnet size is crucial. A subnet mask too narrow will likely miss many potential OpenVPN servers, but a too-broad subnet mask will incur more probing time and may lead to false positives. 

%\input{figures/subnet}

%Figure~\ref{fig:subnet} shows that ..... \DX{pending results}.

\subsection{Test the prober on online University traffic}
To test the specificity of our probing scheme we collected a set of external endpoints visited by clients on our University's IPSec VPN service. For example, if a client with $IP_{A}$ connects to the University VPN at $IP_{B}$ to visit a network service hosted at $IP_{C}$, $IP_{C}$ will be recorded in a database. Our assumption is that the services visited by users while on the university VPN will not be another VPN endpoint. While users from heavily censored regions may chain together VPNs or proxy connections for better security, our university's network is positioned in a country with little censorship restrictions and hence we expect that there are little-to-no chained-VPN cases. We sampled this database on an hourly basis, fetching 1,000 most-visited as well as 10,000 random endpoints visited in the last hour.

%\input{tables/prober-its}

We run this sampling from August 10th 2021 to August 17th 2021, probing the endpoints in batches everyday at 9AM EDT. In total, this results in a dataset of size 2112000 containing 313852 unique IP/port pairs, assumed to be Non-OpenVPN endpoints. Results are shown in Table~\ref{tab:filter-prober}. Overall, 220903 (70.3 \%) endpoints are responsive by the time we send our probes, of which only 37 (0.0167\%) are labeled as ``OpenVPN'' according to our system. 

%\subsection{Summary}


==> related.tex <==
\section{Related Works}
\label{sec:related-works}

\subsection{VPN Detection}
There have been a limited set of previous work focusing on VPN traffic detection. Hoogstraaten~\cite{hoogstraaten2018evaluating} explores the feasibility of detecting proxies and VPN protocols (HTTP proxy, PPTP, SSTP, L2TP, OpenVPN, IPsec, Tor) from the server side. They explored methods ranging from simply using a list of known proxies, and using information databases such as WHOIS and reverse DNS to identify proxies, to exploiting latency and timing as metrics to detect the use of proxies. They also proposed using active scanners send crafted packets to proxy servers and analyzing their responses. 
%\paragraph{Timing Side Channel Techniques}
Webb \etal~\cite{webb2016finding} proposes a proxy detection method based on traffic timing and latency. Their approach relies on the hypothesis that the RTT measurements of traffic when service is accessed by a remote machine through a proxy will be different from the RTT when the service is accessed by the proxy directly. 

%\paragraph{Using ML and NN Models}
Another class of previous works use computational and machine learning models to detect VPN traffic~\cite{VPN-nonVPN, 1d-cnn-vpn, Deep-Packets, perceptron-nn-VPN, VPN-Comparison, LSTM-Attention}. Most of these works use the same \texttt{ISCXVPN2016} VPN-nonVPN dataset~\cite{VPN-nonVPN} to train a variety of machine learning and neural network algorithms. However, we note that the true cost of performing machine learning at line speed remains unclear, and to date, there has been no rigorous study suggesting real-world adversaries deploying ML systems for censorship purposes~\cite{sok-obfs}. Furthermore, previous works used a self-hosted, vanilla OpenVPN to generate VPN traffic for testing. To the best of our knowledge, we are the first to explore the fingerprintability of commercial and/or obfuscated VPN services on real world traffic.


%Random jumble of papers -- bottomline, it is a hard problem.

\subsection{Obfuscation Detection}
%Parrot dead paper

There are research works focusing on the detection of traffic obfuscation tools. Wang \etal examined the fingerprintability of in-use protocol obfuscators such as obfsproxy, FTE, and meek~\cite{detect-obfuscation}. They proposed attacks against these obfuscators using semantics-based attacks, entropy-based attacks, and attacks using machine learning. They conclude that all of the obfuscation mechanisms investigated could be reliably detected by a determined censor. Another team of researchers demonstrate that popular mimicry-based obfuscation tools failed to achieve unobservability because seamlessly simulating another protocol is an extremely challenging task~\cite{Houmansadr2013}. As a result, they were able to use a set of simple passive and active approaches to detect three popular mimicry-based censorship-resistant systems. Previous research papers also suggest that active probing can be used in combination with passive fingerprinting in order to lower the false positive rates. It has been reported that the Great Firewall of China uses active probing in order to block Tor and Shadowsocks~\cite{Ensafi-active-probing, how-china-detect-shadowsocks, how-china-detect-tor}. In response to active probing, ``probe-resistant'' proxies were developed. These proxies remain silent when being probed by an unauthenticated adversary in order to hide their identities. However, researchers were able to demonstrate that even for these proxies, carefully designed active probing could still be effective~\cite{Frolov-probe-resistant}. Our work is inspired by these previous works in designing the \textit{Filters} and \textit{Probers}.


\subsection{Other Traffic Detection Techniques}

Traditional approaches for protocol identification rely on using port numbers. However, it has been shown that such approach could yield very high error rates~\cite{p2p-port, LZR}. Specifically, previous work has found for some popular network protocols, over 97\% servers are not running on the expected ports~\cite{LZR}. Researchers have explored other approaches to identify protocol used in a traffic flow. Sen \etal~\cite{P2P-signature} uses application-level signatures to identify plaintext P2P traffic. By examining documentations of five popular P2P protocols, they compiled a list of signatures and implement a flexible pattern-matching library to detect P2P traffic. For protocol identification over encrypted traffic, pattern matching over packet payload is no longer effective. Instead, flow-level features are used to model the traffic pattern of the tunneled protocol. Bonfiglio \etal~\cite{Skype-Traffic-randomness} proposes a framework based on Pearson's Chi-Square test and a Naive Bayesian Classifier to detect flows that belong to Skype application from a traffic aggregate. Bernaille \etal~\cite{On-the-fly} proposes a light-weight protocol classifier based solely on the size of the first few packets of a given flow. We followed this concept by limiting the inspection of the \textit{Filters} to an observation window, as detecting VPN traffic on the fly is of more interest to ISPs or censors.



%that can be classified as either protocol identification over plaintext traffic ~\cite{P2P-signature, Cute-term-protocol-identification}, or over encrypted traffic ~\cite{Skype-Traffic-randomness, On-the-fly, VPN-nonVPN, 1d-cnn-vpn, Deep-Packets, perceptron-nn-VPN, VPN-Comparison}. Sen \etal~\cite{P2P-signature} uses application-level signatures to identify plaintext P2P traffic. By examining documentations of five popular P2P protocols, they compiled a list of protocol signatures (e.g., \texttt{X-Kazaa-Network: KaZaA}) and implement a flexible pattern-matching library to detect P2P traffic. Yeganeh \etal~\cite{Cute-term-protocol-identification} improves upon a DPI's pattern matching approach with a weighted term matching approach. For example, when a regular-expression uses ``GET.*HTTP'' as a matching signature for HTTP, the proposed system uses ``GET or HTTP'' instead. The authors claim that the proposed term matching system is more flexible and much faster than the traditional approach. %Sen etal - They show that their technique can significantly improve the P2P traffic volume estimates over what a pure port-based approach would provide.

%For protocol identification over encrypted traffic, encrypted payloads make pattern matching no longer effective. Therefore, flow-level features are used as inputs to machine learning algorithms to model the traffic pattern of the tunneled protocol. Bonfiglio \etal~\cite{Skype-Traffic-randomness} proposes a framework based on Pearson's Chi-Square test and a Naive Bayesian Classifier to detect flows that belong to Skype application from a traffic aggregate. %More specifically, the Chi-Square classifier is used to determine which parts of the payload are encrypted and whether the positions of the encrypted parts conform to the Skype protocol. Next, a Naive Bayes classifier is trained on flow-level features such as message size and average Inter-Packet-Gap to learn the underlying traffic pattern of a Skype flow. 
%A highlight of their work is that packet-level features and flow-level features can be complementary, and combining them can potentially lead to better performance and efficiency. Indeed, in this work we followed this idea to complement DPI-based passive fingerprinting with active probing in order to further lower the false positive rates.

%Bernaille \etal~\cite{On-the-fly} proposes a light-weight protocol classifier based solely on the size of the first few packets of a given flow. An advantage of their approach is that, by requiring only the first few packets of a flow, their technique can classify flows on the fly as opposed to identify the flow only when the flow is finished. \TODO{RR: intro this in next section? We followed this idea by attempting to identify a VPN traffic as soon as possible, as from both a censor's and a network administrator's points of view, identifying a VPN traffic can be of limited interest if such identifications can only be done once the flow is finished.}


%although obfsproxy was dev for Tor, others can use it but that is not a good enough fix. There is still data learned by ISP or DPI about timing, and volume of packets, and packet size metrics that can be used to identify and block. CITE China 10 minute window articles/speculations. CITE: entropy and anomaly detection techniques3169 ``OpenVPN'' flows that are potentially false positives

==> tables/dpi-comparison.tex <==
\begin{table}[]
\begin{tabular}{p{2.5cm}|p{7cm}}

Name            & Filter Heuristics \\
\midrule
nDPI & \begin{tabular}[c]{@{}l@{}}
Client Reset and Server Reset Opcodes \\ found in the first two packet\\ (For TCP) first two bytes == entire packet length \\
\end{tabular} \\

Libprotoident & \begin{tabular}[c]{@{}l@{}}
Client Reset and Server Reset Opcodes \\ found in the first two packet\\ (For TCP) first two bytes == entire packet length\\
\end{tabular} \\

Zeek & \begin{tabular}[c]{@{}l@{}}
Client Reset Opcode found in the first packet\\ First packet size matches the expected size \\
\end{tabular} \\

Pang2012OpenVPN & For the first 10 packets of a flow: Client Reset seen once, Server Reset seen once, P\_Control seen at least 4 times, P\_ACK seen at least 3 times \\

This Work      &  \begin{tabular}[c]{@{}l@{}}
Number of different Opcodes is at least 4 \\ but no more than 10\\ The first two Opcodes (Client Reset, Server \\ Reset) not seen after the initial handshake. \\
\end{tabular} \\ 

\end{tabular}
\caption{Comparison of OpenVPN DPI}
\label{tab:dpi-comparison}
\end{table}

==> tables/filter-data.tex <==
\begin{table}[]
\begin{tabular}{|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
\hline
            & ISP Dataset & VPN Dataset \\ \hline
Size        & 461         & 7.65        \\ \hline
Total Flows &             &             \\ \hline
TCP Flows   &             &             \\ \hline
UDP Flows   &             &             \\ \hline
\end{tabular}
\caption{ISP Dataset and VPN Dataset}
\label{tab:filter-data}
\end{table}


==> tables/filter-online.tex <==
\begin{table}[]
\begin{tabular}{|p{0.6\columnwidth}|p{0.28\columnwidth}|}
\hline
Total Bytes Processed  & 11.60 Terabytes  \\ \hline
Total Flows            & 2075 Million  \\ \hline
Flows Exceed Observation Window & 1696420 \\ \hline
%Total TCP + UDP Flows  & 2400 Million \\ \hline
Opcode Filter Positives Count & 6615  \\ \hline
ACK Filter Positives Count   & 4420  \\ \hline
All Positives Count     & 10935       \\ \hline
Positive Rate Over Applicable Flows          & 0.645\%     \\ \hline                   
\end{tabular}
\caption{\textbf{\textit{Filters} test results in the online setting.}}
\label{tab:filter-online}
\vspace{-15pt}
\end{table}

==> tables/filter-prober-combined.tex <==

\begin{table}[]
\begin{tabular}{p{0.1\columnwidth}p{0.48\columnwidth}p{0.25\columnwidth}}
\toprule
\midrule

Filter& Total bytes processed  & 11.60 Terabyte  \\ 
&Total flows            & 2075 Million  \\ 
&Flows $>$ observation window & 1696420 \\ 
&Opcode filter positives count & 6615  \\ 
&ACK filter positives count   & 4420  \\ 
&All positives count     & 10935 (0.64\%)       \\ 
%&Positive Rate Over Applicable Flows          & 0.645\%     \\

\midrule
            Prober&Total Endpoints Probed  & 313852  \\ 
&Non-Connect            & 91385  \\ 
&Failed to complete  & 1564 \\ 
&Total Positives    & 37 (0.016\%)  \\ 
%&Positive Rate          & 0.0167\%     \\ 
        
\midrule
\bottomrule
\end{tabular}
\caption{\textbf{\textit{Filter} and \textit{Prober} test results in online setting}}
\label{tab:filter-prober}
\vspace{-15pt}
\end{table}

==> tables/merit-stats.tex <==
\begin{table}[]
\begin{tabular}{|p{3.5cm}|p{3.5cm}|}
\hline
All Flows  & 23183039736  \\ \hline
Flows longer than Observation Window            & 10070994  \\ \hline
Flows after filters  & 75850 \\ \hline
Flows after probers & 3638  \\ \hline
VPN rate over applicable flows    & 0.0361\%  \\ \hline
\end{tabular}
\caption{Statsitcs of testing results from Merit}
\label{tab:merit-stats}
\end{table}

==> tables/prober-its.tex <==
\begin{table}[]
\begin{tabular}{p{3.5cm}|p{3.5cm}}
\toprule
\midrule
Total Endpoints Probed  & 313852  \\ 
Non-Connect            & 91385  \\ 
Failed to complete  & 1564 \\ 
% Explicit OpenVPN ServerHello & 1111111111  \\ \hline
% I didn't collect this bit of information, sorry! I don't think it adds much to the table, compared with total positives anyway.
Total Positives    & 37  \\ 
Positive Rate          & 0.0167\%     \\ 
\midrule
\bottomrule
\end{tabular}
\caption{\textbf{\textit{Prober} test result on online University traffic.}}
\label{tab:prober-its}
\vspace{-15pt}
\end{table}
